Learning task-agnostic representation via toddler-inspired learning

One of the inherent limitations of current AI systems, stemming from the passive learning mechanisms (e.g., supervised learning), is that they perform well on labeled datasets but cannot deduce knowledge on their own. To tackle this problem, we derive inspiration from a highly intentional learning system via action: the toddler. Inspired by the toddler's learning procedure, we design an interactive agent that can learn and store task-agnostic visual representation while exploring and interacting with objects in the virtual environment. Experimental results show that such obtained representation was expandable to various vision tasks such as image classification, object localization, and distance estimation tasks. In specific, the proposed model achieved 100%, 75.1% accuracy and 1.62% relative error, respectively, which is noticeably better than autoencoder-based model (99.7%, 66.1%, 1.95%), and also comparable with those of supervised models (100%, 87.3%, 0.71%).

==> Sections-backup/0_Abstract.tex <==
\begin{document}

%Although deep learning methods have achieved remarkable performance in various vision tasks, those require large amount of well-labeled data and still prone to noise and change of perspective. For instance, . In contrast, toddlers seems to have the ability to rapidly learn those features only with few objects weak supervisions. It seems that there exists some fundamental difference between human learning and current AI learning.
One of the inherent limitations of current AI systems, stemming from the passive learning mechanisms (e.g., supervised learning), is that they perform well on labeled datasets but not able to deduce knowledge on their own. 
The field of deep learning-based computer vision is no exception, and
%One of the intrinsic limitations of current AI systems, stemming from the passive learning mechanisms (e.g., supervised learning), is that they require large amount of labeled data sets and hard to extrapolate its knowledge to other tasks. However, toddler  obviously  has the  striking  ability  to  learnthose features only with few objects without explicit labels.
how human obtains extrapolatable knowledge from visionary tasks without any given labels still remains a question.
%who have the innate cognitive mechanism, produce and even  
To help address this, we derive inspiration from a highly intentional learning system via action: the toddler. 
%Inspired by the toddler's learning procedure, we design a virtual environment where the agent can explore and interact with objects.
Inspired by the toddler's learning procedure, we design an interactive agent which can learn and store task-agnostic visual representation while exploring and interacting with objects in the virtual environment.
%To make the agent learn the understanding of objects from its interaction, we designed the agent to store those understandings as an interaction feature map.
Experimental results show that such obtained representation was expandable to various vision tasks such as image classification, object localization, and distance estimation tasks. In specific, the proposed model achieved
100\%, 75.1\% accuracy and 1.62\% relative error, respectively, which is noticeably better than autoencoder-based model (99.7\%, 66.1\%, 1.95\%), and also comparable with those of supervised models (100\%, 87.3\%, 0.71\%).
%e.g. 100\%, 98.9\%, 82.5\% relative accuracy compared to supervised methods in image classification, distance estimation and object localization
%One of the intrinsic limitations of current AI systems, stemming from the passive learning mechanisms (e.g., supervised learning), is that they require large amount of labeled data sets and hard to extrapolate its knowledge to other tasks. In constrast, toddler obviously has the ability  to  learnthose features only with few objects without explicit labels.\
%Then, how human being extrapolate their knowledge without any given labels still remains a question.
%To help address this question, we derive inspiration from a highly intentional learning system via action: the toddler. In this work, we propose a basic set of tasks that require toddler agents to classify the three objects: Ball, Rattle, and Doll, without any given labeled data in the frame of the way toddler learns. Our experiment goes on the VECA environment: A VR Toolkit for Training and Testing Cognitive Agents. In specific, we design a navigation task that takes account of the agent's intention and rewards the agent if the navigated object matches the intended object. We observe that the agent was able to gain an expandable understanding of those objects during navigation, and those understanding were more robust compared to supervised methods.
\end{document}


==> Sections-backup/1_Introduction.tex <==
%\documentclass[../draft.tex]{subfiles}
%\begin{document}

\section{Introduction}

%Although deep learning methods have achieved remarkable performance in various vision tasks, those require large amount of we;ll-labeled data and still prone to noise and change of perspective. For instance, . In contrast, toddlers seems to have the ability to rapidly learn those features only with few objects weak supervisions. It seems that there exists some fundamental difference between human learning and current AI learning.
Recent deep learning methods have significantly outperformed previous state-of-the-art algorithms in the computer vision domain by learning to capture intrinsic feature structures of the large-scale data~\cite{voulodimos2018cvsurvey}. 
%~\cite{Deep Learning for Computer Vision: A Brief Review}
%robotics, video games, health care, and else. 
Still, there are two major discrepancies between human learning and current data-driven learning, especially supervised learning-based ones. 
%However, general, there are two major limitations 
First, a well-distributed large labeled dataset is needed to learn a feature properly~\cite{DBLP:journals/corr/abs-1811-06052}. Second, they are task-specific in the sense that adapting to multiple different tasks or transfer learning is difficult~\cite{lake2017buildingmachines}.
%First, well-distributed large labeled dataset is needed to learn a feature properly~\cite{DBLP:journals/corr/abs-1811-06052,into2015surpassing}. Second, they are task-specific in the sense that adapting to multiple different tasks or transfer learning is difficult.
%:  machine learning generally still compared with the human child's learning system owing to the different mechanisms of learnin}. 
%For instance, in the vision-based task, some machine learning models have reached superior performance only when they tune a large amount of well-labeled data sets for the specific task.
%From the existing mechanism of machine learning, there are

%Several methodologies like semi-supervised learning, meta-learning or meta-learning aim to improve task generality and data efficiency.
Several methodologies like semi-supervised learning, meta-learning or multi-task learning aim to improve task generality and data efficiency.
However, they assume that prior tasks are well-labeled and easily trainable, which are limited in solving both problems.
%Attempts to narrow this gap, like multi-task learning, meta-learning, or data augmentation, still have limitations in solving both the problem.
These discrepancies stem from the difference in how human and data-driven AI models the learning~\cite{lake2017buildingmachines}. 
A solution could be found by investigating the learning process of human and integrating it into AI techniques. 
%Supervised learning-based methods take a statistical approach, whereas humans build a generalized model of the task with few data observations. 
%of data, so it is much sensitive to the data distribution of the given dataset and task. So it lacks task generalization and data inefficiency 
%These intrinsic limitations are due to the top-down learning approach; Existing machine learning, 
%requiring the completed labeled data sets before they start learning the domain of knowledge, sets in the reverse process of bottom-up learning approach embedded in human. This reverse mechanism of ML brings the increase of task-dependency and prohibits the current AI from reaching the level of human intelligence. 

%Toddler obviously has the striking ability to learn those features only with few objects without explicit labels. How could toddlers gain a general understanding of objects without any explicit labels? We have to focus on how child learning clearly uses a different mechanism of learning trained from the blank sheet to the mature domain of knowledge rather than ML mechanism.
%The necessity of applying the child learning approach when we design the machine also has been proposed by Turing~\cite{turing2009child}, who pointed out that figuring out how the child learns is the key in order to jump on the next human-level-intelligence. Hence, we draw inspiration from the child(toddler) to understand how their bottom-up learning approach is working without any explicit well-labeled data. 
%We think that one of the major difference between two learning methods is activeness.

%Along with this, one of the other interesting theories about Toddler's understanding is the theory suggested by Piaget\cite{piaget1952origins}, which argues that the infant's understanding of objects is centered on actions. For example, when a toddler sees a wooden ball, she doesn't know what is it yet. However, the toddler does various actions (e.g., rolling, punching) to the ball, and she gains the information with these actions (e.g., This object is rollable, it makes me hurt when punched). Although this is not a perfect interpretation of 'wooden ball', she can gain a general understanding of it such as rigidness.
%In this paper, we try to connect human learning to AI learning. 
%In this paper, our goal is to , inspired . 
In this paper, we seek a new approach to overcome aforementioned limitations inspired by a highly intentional learning system via action: the toddler. Researchers in AI have been
taking an interest in learning of a child to seek technical advances~\cite{bambach2018toddlerinspiredvisualobject,schank1972nlp,turing2009child}. Developmental psychologists have studied in a large scale that general understanding of objects develops in an early stage of the toddler without any supervision, through interaction on objects like mouthing, chewing, and rotating~\cite{gibson1988toddlerlearning,piaget1952origins}.
%Toddler acquires such abilities through interaction on objects like mouthing, chewing, rotating. 
%For example, when a toddler encounters a wooden ball for the first time, the toddler inspects it with various actions (e.g., rolling) and understand properties of it, such as rigidness.
%This raw sensory-perceptual feedback facilitates cognitive development.
%, and proceeds to more sophisticated interactions like talking to a toy phone. 
We believe that the toddler-inspired learning procedure can nurture task-agnostic knowledge of objects by exploring and interacting with the environment, and it will be the key to overcome limitations of supervised learning.

%It gives an inspiration that toddlers acquire task-agnostic knowledge through interaction-based exploration of the environment and use that knowledge to adapt to the newly encountered task or learn a new object with few observations via prior knowledge.
%We believe that toddlers acquire task-agnostic knowledge through the initial random exploration of the environment and use that knowledge to adapt to the newly encountered task or learn a new object with few observations via prior knowledge.
%We believe that referring to toddler's learning procedure could be the promising direction to overcome current limitation of AI systems.
%We believe that developing toddler-inspired learning procedure, which can acquire general understanding of objects without any supervision via interaction-based exploration, could be a key to overcome limitations of current AI systems.
%We believe that toddler's learning procedure is a key to acquire , which could be a key to overcome current limitation of AI systems.

%In this light, we propose a novel toddler-like learning procedure, which aims to gain understandings of objects without explicit labels, by exploring and interacting with the environment as a toddler does.
%To take the first step on the framework of the toddler-inspired learning, we try to roughly simulate one major component of toddler learning procedure: exploration. In specific, we designed an environment in which the agent can walk around and interact with objects, and let the agent explore the environment. After the exploration, we try to extrapolate its knowledge via transfer learning to other computer vision tasks: image classification and depth estimation, in order to show the adaptation of new knowledge from a prior one. We observed that transferred models were able to achieve comparable performance with supervised methods, which indicates that the agent was able to gain an expandable understanding of objects during exploration and interaction.

%As a first step on the framework of the toddler-inspired learning, we try to roughly simulate toddler's one of the early learning procedure, which acquire task-agnostic knowledge through exploring and interacting with its surrounding environment.
%In this light, we would like to take a first step on the framework of the toddler-inspired learning by roughly  simulate toddler’s early learning procedure. 
%To take the first step on the framework of the toddler-inspired learning, we try to roughly simulate one of the toddler’s early learning procedure:  exploring and interacting.
As the first step in developing toddler-inspired learning procedures, we simulate the interaction-based learning of a toddler. In particular, we first designed a virtual environment where the agent can freely roam and interact with objects and gets feedback (reward). Second, we designed the agent's network architecture to extract the understanding of objects based on interactions and store those understanding in \emph{interaction feature map}. Interaction feature map is designed to have only one feature image per interaction to make the agent learn a compact interaction-based representation.
%To be more specific, interaction features consists of one feature map for each available interaction of the agent, which requires the agent to learn a compact interaction-based representation.
%To be more specific, we designed interaction features to have only consists of one feature map for each available interaction of the agent, which requires the agent to learn a compact interaction-based representation.
% We propose a novel architecture which can store interaction-based understanding of objects during exploration, like toddler learns.
%We designed the agent to store the interaction-based understanding of objects as a feature map for each interaction, and let the agent explore the environment.
%After the exploration, we show that the acquired visionary knowledge could be extrapolated to several computer vision tasks through transfer learning.
%We let the agent explore the environment and show that the acquired visionary knowledge could be extrapolated to several computer vision tasks through transfer learning.
We let the agent explore the environment and transfer its acquired visionary knowledge to several computer vision tasks by connecting additional layers to learnt interaction feature map.
%try to extrapolate its knowledge via transfer learning to other computer vision tasks in order to show the adaptation of new knowledge from a prior one.
%Despite the fewness of interaction features, transferred models were able to achieve 99.7\%, 62.8\% accuracy and 3.0\% relative error in image classification, object localization task and distance estimation, comparable to supervised models which achieved 99.7\%, 76.1\% and 1.9\%. It indicates that the agent could gain an expandable understanding of objects during interaction-based learning.
Even though the number of feature images in interaction feature map is extremely small, transferred models were able to achieve 99.7\%, 62.8\% accuracy and 3.0\% relative error in image classification, object localization task and distance estimation, comparing to those of supervised models, 99.7\%, 76.1\% and 1.9\%. It indicates that the agent could gain an expandable understanding of objects from interaction-based learning.
%such as image classification, object localization, and distance estimation tasks, and achieved 99.7\%, 62.8\% accuracy and 3.0\% relative error, respectively, comparing to those of supervised models, 99.7\%, 76.1\%, and 1.9\%.
%Transferred models were able to achieve 100\%, 98.9\%, 82.5\% relative accuracy compared to supervised methods in image classification, distance estimation, and object localization task, which indicates that the agent can gain an expandable understanding of objects during interaction-based learning.

%Inspired by Piaget's theory, we would like to see whether understanding of objects could be gained during exploring and interacting with the environment, and also could be extrapolated to other tasks. So we designed an environment in which the agent can walk around and interact with objects, and let the agent explore the environment. After the exploration, we try to extrapolate its knowledge via transfer learning to other computer vision tasks. We observed that transferred models were able to achieve comparable performance with supervised methods, which indicates that the agent was able to gain an expandable understanding of objects during exploration and interaction.
\iffalse
Contributions of our paper are summarized as follows :

\raggedbottom
\begin{itemize}

    \item We introduce a new learning procedure inspired by how toddlers learn to overcome two major limitations of supervised learning : data inefficiency, task specificity.
    
    \item We organized a Unity3D-based virtual simulation of toddler-like learning procedure, and experimented~

    \item We 

\end{itemize}
\fi
%\end{document}


==> Sections-backup/2_Background.tex <==
\section{Background}

\subsection{Related works}
%\hs{Where is current SOTA RL heading? What is the difference of current RL and human intelligence, and the limitation from it?}
%Deep reinforcement learning(DRL) applies deep learning techniques in reinforcement learning framework, showing a great performance in various domains like game theory, optimal control and multi-agent system. Representative algorithms leading these advances are Policy gradient and Deep Q-learning methods.
 % what are the cons of supervised learning?
 % What are the pros of human-like learning / toddler-like learning?
 % Human-like machine learning: limitations and suggestions


%Supervised learning has fundamental limitations in reaching the level of human intelligence despite its advances in fields like computer vision. Firstly, it requires a huge well-labeled dataset to learn a concept or a task, whereas a human can learn with few observations~\cite{lake2017buildingmachines}. It works on the assumption that the dataset is representative, large enough and covers all possible cases~\cite{DBLP:journals/corr/abs-1811-06052} which is in some cases impracticable in domains like medical imaging or activity recognition. Moreover, supervised learning-based algorithms are highly task-specific in the sense that they are optimized well for a single task, but gets trouble in solving multiple tasks~\cite{lake2017buildingmachines}. An agent should at least be able to fit similar tasks with little data to reach the level of artificial general intelligence(AGI). 

%\hs{What is a current limitation of RL, and AI broadly, which will need a human-like learning point-of-view to solve it?}

\iffalse
\textbf{Transferring methods.}
e.g. Meta-learning, Transfer learning, domain adaptation
Need tasks that are in similar domain, well-labeled, easily trainable.

\textbf{Unsupervised methods.}

e.g. XXX-Autoencoder, k-means
Does not work well : lack of inductive bias = poor representation(no difference with compression)
\fi

Attempts to narrow these major discrepancies 
cannot alleviate both of them due to their own limitations. 
Semi-supervised learning trains the predictor given both the labeled data and extra unlabeled data to reduce the cost of labeling.
However, theoretical analysis has found that it increases sample complexity only by a constant factor compared to supervised learning without strong assumption on unlabeled data~\cite{lu2009semisupervisedlearning}.
%suggestive links to the learning in psychology
%~\cite{botvinick2019RLfastandslow}. 
%Data augmentation,
%Simulation-based data synthesis
%Episodic memory, storing records of past events and reusing it to overcome the sample inefficiency, resembles instance-based theories of learning in psychology.
%multitask learning,
% Need to 
%~\cite{logan1988instancebased}.
%In particular, meta learning, term originated from 'learning to learn' in psychology,~\cite{harlow1949learningtolearn}
Meta-learning trains in a set of tasks (usually well-known or general) and leverages the acquired knowledge or configuration in learning a similar task. 
%It does not solve the limitation of supervised learning because there should be sufficient number of well-labeled prior tasks much similar to the target task~\cite{kang2018transferablemetalearning}. 
Still, there should be a sufficient number of well-labeled prior tasks much similar to the target task~\cite{kang2018transferablemetalearning}.
Multi-task learning effectively adapts to a set of related tasks simultaneously by forming an inductive bias from intrinsic dependencies of tasks, but it is difficult to optimize shared parameters in competing objectives of each task~\cite{liu2019multitasklearningauxilarytask}.
%Also, prevailing model-agnostic meta learning(MAML) approaches even assumes simple and concentrated prior task distribution~\cite{vuorio2019multimodalmaml}, which needs further supervision of the developer.

%autonomous learning,

%Semi-supervised learning, self-supervised learning, unsupervised learning, task-agnostic reinforcement learning

%Term was introduced from a psychology domain, that a strong prior knowledge learnt from a specific task are applied in learning a new related task. 
% reward plane 이 gradient descent 에 의해서 수렴이 보장되는 (convex느낌) 걸로 해야된다
% sample inefficiency
% 아키텍쳐간의 비교 : 옆에 supervised 붙이는 아키텍쳐랑 그냥 rl input으로 두 이미지 concat해서 넣은 다음에 intention 없이 줘서 알아서 intention 형성되게하는 구조 
\subsection{How Toddlers Learn}
%Even though recent biologically inspired advances in AI prevails in tasks which were thought only for the human, they are

%\hs{What is a human-like learning and why do you need human-like learning to solve current limitations?}

%\hs{Why can the human-like learning provide a breakthrough to these limitations that other approaches like meta-learning cannot?}
To 
%overcome the limitations of supervised learning and 
build a machine that learns like a human, we need to fuse the human learning process to current AI techniques.
There is a basic difference between data-driven AI and human intelligence in the model of how they learn~\cite{lake2017buildingmachines}. Data-driven AI takes a statistical pattern recognition-based approach, so the accumulation of knowledge relies on the observed data. 
% Prof.Zhang paper i have cited below
In contrast, human actively inspects the environment to collect data and learns with only a few of it by building a generalized model of the world.% to understand them. %~\cite{lake2017buildingmachines}.
%Human-like learning~\cite{DBLP:journals/corr/abs-1811-06052} introduced bio-inspired self-driven data collection in simulation environment to overcome data availability issue in activity recognition. 
%Another attempts tried to mimic human cognition by building an artificial theory-of-mind~\cite{winfield2018TOMexperiments,rabinowitz2018TOMNet,gorur2017TOMSocialRobot} which is the ability to attribute mental states (intentions, desires) of others. However, they was criticized for simplifying the cognitive task into merely a behavioral prediction, rather than actually attributing mental states of others~\cite{shevlin2019PsychologyTermsinAI}.

%, and should take care when analyzing artificial intelligence in an psychological perspective .

% Byungtak Jhang. 2018. Human Intelligence and Machine Intelligence: Cognitive Artificial Intelligence (in Korean). Communications of KIISE 36, 1 (2018), 17–26.
% How do we cite this korean article?
%A promising direction to overcome such differences is constructing cognitive agents that imitate human-like perceptions and mental process. some works report that cognition is highly correlated with performing actions and having rich perceptions. Reflecting how human learn, cognitive agent aims at learning task-independent knowledge by continuously observing environment with various sensory perceptions and solving generic tasks. There have been early discussions in robotics and computer science of building cognitive agents~\cite{lee2017cognitiveagentearlywork}.

The learning process of a child is important for learning-to-learn capabilities like goal-setting, self-control~\cite{zosh2017learnthruplayreview}, and should be taken into account in developing AGI. Life experiences and prior knowledge learnt in childhood are known to influence the learning of a grown-up.
%Importance of childhood learning has thus raised attention to computer scientists like Turing or Schank~\cite{turing2009child,schank1972nlp} aiming to model the AGI. 
%Instead of building a machine imitating adult mind, Turing suggested to build a child mind and educating it~\cite{turing2009child}. Schank has also made a prospect of a program expanding their knowledge like a child, instead of catered in tremendous data~\cite{schank1972nlp}.
The latest works in deep learning like visual object learning~\cite{bambach2018toddlerinspiredvisualobject} 
%or few-shot learning~\cite{ritter2017cognitivepsyonDNN} 
are seeking advance from how children learn. 
%Data collected from toddler-like visual system is used to train visual object learning better, or one-shot learning image classification model shows a similar shape bias as children.

%\hs{What is the difference of toddler and adult human being and what can be inspired from the toddler's learning?}
Researches in developmental psychology suggest that toddler unconsciously learns through interaction and play with their surrounding environment, rather than self-directed task-specific learning of an adult~\cite{mcdonough2013difference_adult_child}. Too early the start of formal subject teaching for a child is known to be counterproductive and hinders academic performance in the long run~\cite{suggate2013childlatelearning}. Instead, it is universally accepted that children learn cognitive or self-regulatory abilities by playing~\cite{piaget1952origins,zosh2017learnthruplayreview}.
%Piaget viewed that toddler builds much abstract and symbolized model of the surrounding world through playing.
%, and a new kind of psychological functioning emerges.
%playing increases in the developmental stage of a toddler (preoperational stage) in order to~\cite{piaget1952origins}.
%However, playing of toddler is usually not self-directed, but more like a random interaction with the environment.
%Adult learners have more self-directed nature of learning process to formulate a learning goal due to their prior knowledges whereas child learners is less self-directed and more unconscious of their learning process~\cite{mcdonough2013difference_adult_child}.
Large-scale studies on exploratory object manipulation in early childhood has found that changes from random actions on objects to more self-directed and functional activities happen at the latter part of the first years of a child~\cite{gibson1988toddlerlearning}. Random actions in the early exploration are suggested as investigating an object with the raw sensory-perceptual feedback, with visuotactile inspection like mouthing, chewing, rotating, banging and else. These activities promote the development of cognitive capacities and control and progress to more functional and imaginative plays like talking to a toy telephone. It gives an inspiration that action-based exploration of a toddler can facilitate an unsupervised categorization of the objects, and furthermore, help gain a general knowledge of the world that can be used to adapt to a specific task.

%both adults and children need to use the learning or employ the knowledge gained. The more the knowledge is used, the closer the approximations come to the conventions and become internalized. Feedback to both the adult and the child helps each learner fine tune the approximations. Once the learning has been internalized, the knowledge is transferred into new situations by both the adult and child learners. A major characteristic that impacts the natural learning process is engagement of both adult and child learners. The more actively engaged in the learning process, the faster the knowledge is obtained and the better the knowledge is learned. 
% 이부분정리해야함
%In the 1970s the literature of early childhood was enriched by large-scale studies of exploratory manipulation of objects (e.g. McCall 1974; Fenson et al 1976). The relevant concept that inspired these studies was cognition, as the study of cognitive development emerged with the new focus on cognitive psychology. Emphasis was placed on a change toward the end of the first year of a child's life from relatively random action on objects, to cognitively directed "functional" activities, such as drinking from a toy cup or talking into a toy telephone instead of banging them on somelhing. McCall suggested that early exploration was "largely an investigation of the raw sensory-perceptual feedback of the objects" (1974, p. 77), which changed progressively toward greater cognitive control and imaginative play with the object. Fenson et al (1976) similarly stressed emergence of new "cognitive capacities" following nonspecific manipulation: Although 9-month-olds generally showed the ability to relate to objects and 7-month-olds did not, at both ages play was nonrelational and nonaccommodative and was characterized by close visual and tactual inspection of individual objects, usually accompanied bymouthing and chewing and the application of more or less indisciminate motor schemes
%(shaking, banging, turning the object over and over, and shifting it from hand to hand) ....The emergence of relational acts in the latter part of the first year and the emergence of symbolic acts in the first half of the second year dramatically change the structure of the child's play, mirroring the development of important new cognitive capacitis (pp. 234 ff).It is interesting to read that the play mirrors the development of new cognitive capacities, rather than that the manipulative play has a key role in cognitive development, as Piaget would have suggested. 

%\hs{What are you actually trying to do? formulate it clearly please.}
%world exploration

%\hs{How does this represent the human-like learning?}
%\hs{How is it different from meta-learning?}
%\hs{What is the problem and why are you trying to solve in this way?}
%\hs{How is human-like learning applied in your implementation? }
%\hs{ Why are you using a navigation task to demonstrate the human-like learning?}


==> Sections-backup/3_Methods.tex <==
\section{Methods}
\textbf{Interactive Virtual Environment.}
%To train the agent without any explicit labels, 
Motivated by~\cite{gibson1988toddlerlearning}, we designed an environment supporting the human-like visual observation and active physical interaction with the object, to train the visionary knowledge prior without any explicit labels.  We used VECA~\cite{VECA}, a virtual environment generation toolkit for human-like agents, to implement the environment. Reward structure of the environment provides a sparse positive reward signal when the agent is touching or playing with the prop objects, and near-zero negative reward is given to aid the navigation to the prop object. With this reward structure, the agent is motivated to visually locate far objects when it is freely exploring and observe an interacting objects in depth when it is nearby. The agent  collects data without any label and establishes a deeper visual understanding of an object, compared to the unsupervised learning on object images without any context.
\iffalse
that includes 3 objects (toy pyramid, ball, doll) and a baby agent.  which supports realistic observation and action, to implement this environment.
The agent receives RGB 84x84 binocular vision and has two kinds of action - movement(walk) and interaction(hold, kick, press). The movement of the agent is represented as a two-dimensional vector (walking velocity). The agent is rewarded when the agent successfully navigated to the object and interact with the object. The reward is determined for each object-interaction pair, which could be positive (If the baby presses the doll, then the doll will make sound and baby will be joyful) or negative (If the baby kicks the toy pyramid, then the baby will feel pain).
\fi

\textbf{Toddler-inspired learning.} 
%In the long run, we aim to develop a toddler-like learning procedure, which can acquire a general understanding of objects without any supervision by exploring and interacting with its surroundings. As the first step, we designed a toddler-inspired learning procedure as shown in Fig. \ref{figure:Overview}. In the training procedure, the agent learns visual transferable knowledge by exploration and interaction without any explicit label given. The agent is tested by the generality of the knowledge, which is evaluated as the transferability to three vision tasks: image classification, distance estimation, and object localization.
With the interactable environment, we formulate the toddler-inspired learning framework, which aims to acquire a general understanding of objects without any supervision, but by exploring the environment and interacting with the objects, as toddler does. 
We assume that the agent can only visually observe and interact with the object during the sparsely rewarded reinforcement learning task. With the reinforcement learning, we want the agent to learn a transferable representation embedding $f_{\theta}(x)$ parameterized by $\theta$ through sufficient observation and interaction, without any supervision of the downstream tasks. The representation mapping $f_{\theta}(x)$ will be used as a general prior for supervised downstream tasks $\mathbb{T} = \{T_i\}_{i = 1,\cdots,n}$ with datasets $\mathcal{D}_{\mathbb{T}} =\{\mathcal{D}_{T_{i}}\}$
%,$ D_{T_{i}} = {(x_j, y_j)}$ %\{(\mathcal{X}_{T_{i}}, \mathcal{Y}_{T_{i}})\}$
%_{i = 1,\cdots,n}
collected from the environment. 

The framework consists of two phases. First, the transferable representation $f_{\theta}$ is pretrained in an interactable environment, by solving a reinforcement learning problem in Eq. 1. $o_t$, $a_t$ represents observation, action in time $t$, while $r(\cdot)$, $\pi_{\psi}(\cdot | \cdot)$ and $\gamma$ are reward function, policy and discount factor, respectively. Second, we use the representation mapping $f_{\theta}(x)$ as an embedding prior and transfer learn the downstream tasks $\mathbb{T}$. We evaluate the generality of representation with its transferability, which results in maximizing the sum of each objectives shown in Eq. 2. and $\{J_{T_i}\}$ denotes the set of objective function for each task $\{T_{i}\}$. Please note that we can't directly optimize the formula since the task distribution is unknown while training.
\begin{align}
%\textrm{Maximize} ~~ J_{train}(f(\cdot)) = \sum_{t=0}^{\infty} {\gamma}^t r(s_t, \pi_{\psi}(a_t|f_{\theta}(o_t))) \\
\hat{\theta}, \hat{\psi} = \argmax_{\theta, \psi}J_{train}(f_{\theta}, \pi_{\psi}) = \argmax_{\theta, \psi} \sum_{t=0}^{\infty} {\gamma}^t r(s_t, \pi_{\psi}(a_t|f_{\theta}(o_t))) \\
\textrm{to indirectly maximize} ~~ J_{test}(z) 
= \sum_{T_i \in \mathbb{T}} \sum_{(x,y) \in \mathcal{D}_{T_{i}}} J_{T_i}(f_{\hat{\theta}}(x), y)
\end{align}
Fig. \ref{figure:Overview}. shows the overview of the procedure in our toddler-inspired learning framework. In the first phase, the agent trains under the reinforcement learning framework and learns the efficient transferable representation, which we named as \emph{interaction feature maps}, through exploring the environment and interacting with the object. In the second phase, the representation embedding is used as a feature extractor of the data points on downstream tasks. In this figure, the generality of the representation embedding is evaluated with the transferability to three vision tasks: image classification, distance estimation, and object localization.

%To show that the agent could acquire transferable knowledge from the environment, we measured the generality of the knowledge with its transfer performance.
%In specific, we fixed the parameters of the agent and connected linear layers to the interaction feature map.
%We evaluated the performance with three vision tasks: image classification, distance estimation, and object localization.

%In the long run, we aim to develop a toddler-like learning procedure, which can acquire a general understanding of objects without any supervision by exploring and interacting with its surroundings. As the first step, we designed a virtual environment with interactable objects where the agent freely explores and interacts with the objects. 
%To enable the agent to learn understanding of objects from interaction and store them in a compact form, we designed the agent to store those understanding as \emph{interaction feature maps}.


%As toddler's early understanding of objects is based on its interaction,We designed the agent to store the understanding of objects as a feature map corresponding to each interaction.
%Like toddler's learning, we would like to let the agent interact with the environment motivated by its intrinsic reward. However, designing toddler-like robust intrinsic reward function itself is definitely a challenging task. To detour this problem, we limited the number of object and interaction and hand-crafted the reward for each pair of object and interaction. We suggest that developing robust intrinsic reward function and substituting hand-crafted reward with those reward function could be a promising future direction.

\iffalse
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.4\textwidth]{Pictures/fig0_2.png}
    \caption{Snapshot of the VECA environment.}
    \label{figure:Environment}
\end{figure}
\fi

%Inspired from toddler's learning procedure, we want to see whether understanding of objects could be gained during exploring and interacting with the environment, and also could be extrapolated to other tasks. So we designed an environment where the agent can walk around and interact with objects, and let the agent explore the environment. After the exploration, we tried to extrapolate its knowledge to other computer vision tasks.

%\subsection{Environment for toddler-like learning}

%To , we designed a toddler-like navigation task. The environment is a room which have 3 objects (rattle, ball, doll) and baby agent inside. This task consists of two parts - navigation and interaction. In the navigation part, agent must navigate the s. We reward the agent when the baby finish the navigation.

%Inspired by toddler's dhlrus, we designed an envrionment which the agent can walk around and interact with objects.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Pictures/WOverview_v2.png}
    \caption{Overview of  toddler-inspired learning framework and network architecture. 
    %The observation is encoded as an \emph{interaction feature map} with CNN \& MLP encoder. In the training process, the interaction feature map is masked with intended interaction and fed to MLP, which outputs state value function $V(s)$ and movement policy $\pi(a|s)$. In the testing process, we transfer the \emph{interaction feature map} to various tasks. Best viewed in color.
    }
    \vspace{-10px}
    \label{figure:Overview}
\end{figure*}


%We designed an environment which includes 3 objects (toy pyramid, ball, doll) and a baby agent, as shown in \ref{figure:Environment}. We use VECA~\cite{VECA}, which supports realistic observation and action, to implement this environment. The agent receives RGB 84x84 binocular vision and have two kinds of action - movement(walk) and interaction(hold, kick, press). Movement of the agent is represented as a two-dimensional vector, which corresponds to the walking direction. The agent is rewarded when the agent successfully navigated to the object and interact with the object. The amount of the reward is determined for each pair of object and interaction. It could be positive (If the baby presses the doll, then the doll will make sound and baby will be joyful), or negative (If the baby kicks the toy pyramid, then the baby will feel pain). We expect the agent to learn the mapping between its desired interaction and its visual perception, which naturally requires to learn about concepts of objects. We suppose that the agent has an intention to do certain interaction during the exploration, and tries to maximize its reward.

%The environment is a room consists of 3 objects (toy pyramid, ball, doll) and a baby agent. The agent have two kinds of action - movement(walk, turn) and interaction(hold, kick, press). The agent is rewarded when the agent successfully navigated to the object and interact with the object. The amount of the reward  each pair of object and interaction . We suppose that agent has a fixed 'intended interaction' during navigation. Thus, the agent has to learn the mapping between its desired interaction and object, such as "ball is a kickable object".

%\subsection{Learning from free exploration} 

%\textbf{Network Architecture for Interaction-based Learning.} 
%We designed the architecture of the agent as Fig \ref{figure:Agent}. Inspired from RDCNN~\cite{xue2019image}, we designed the encoder as a fixed random-weight depthwise CNN with sign activation, where we found it significantly accelerates the training. Output feature maps of the encoder are linearly combined to make interaction features. To make interaction features to store interaction-based features of the object, we designed the network corresponding to its interaction the interaction feature map is masked with intended interaction.Since the movement of the agent only depends on interaction features, each feature map must learn to represent abstract features of the object corresponding to its interaction.

\textbf{Network Architecture.} To learn and store transferable knowledge, we designed the architecture of the agent as Fig.~\ref{figure:Overview}. Visual observation of the agent is encoded with CNN and MLP, resulting in \emph{interaction feature maps}. 
Those feature maps are masked with linearly embedded intention, and determines the action of the agent.
Since the movement of the agent only depends on masked features, the agent must learn to represent abstract features of the object corresponding to its interaction.

%\textbf{Training.} We supposed that the agent has an intention to do certain interaction and tries to maximize its total reward. We formulated this environment as a reinforcement learning task and used SAC~\cite{haarnoja2018soft} to train the agent. Please note that developing a human-like training algorithm is not the focus of this paper, rather we focus on the learning task itself. We agree that developing human-like fast and adaptive learning algorithm is a challenging and important problem, and suggest that those could be discussed for future works.

%For evaluation experiments, we train a linear layer connected to the action features (Highlighted with yellow dotted lines in \ref{figure:Agent}). We used softmax activation for image classification. Additionally for image classification, we design a self-supervised model which could be trained while navigating the environment by using intention as a label. We evaluate this model directly without additional training to evaluate whether action features contains the feature to the corresponding intention. Please note that this classifier doesn't learn from inaccessible supervision(which gives a major difference with supervised classification), and almost 30\% of the observation are heading to the wall even the agent converged to the optimal policy (which indicates that intention is not a well-shaped supervision). To mitigate the noisy observation, We maintain a replaybuffer with size of 50000 and train with those data. Also, we apply label smoothing and PPO-like ratio clipping to stabilize the training. 


==> Sections-backup/4_Experiments.tex <==
\section{Experiments}

\subsection{Experimental Setup}
%To evaluate the generality of knowledge gained during exploration, we measure the transfer performance with other vision tasks.
%To evaluate our proposed learning procedure, we measured the generality of knowledge gained during exploration with its transfer performance.
To show that the agent could acquire transferable knowledge through the toddler-inspired learning framework, we evaluated the transfer performance of the interaction feature map on three  supervised visionary downstream tasks: image classification, distance estimation, and object localization.
In specific, we fixed the parameters of the interaction feature map $f_{\theta}$ after pretraining and connected linear layers for transfer leanrning.
We used VECA~\cite{VECA} toolkit to  implement an interactive 3D environment that includes 3 prop objects (toy pyramid, ball, doll) and a baby agent. The agent receives RGB 84x84 binocular vision and has two kinds of action - movement and interaction(hold, kick, press). 
%The movement of the agent is represented as a two-dimensional vector (walking velocity). The agent is rewarded when the agent successfully navigated to the object and interact with the object. 
The reward signal is designed for each object-interaction pair. It could be positive (If the baby presses the doll, then the doll will make sound and baby will be joyful) or negative (If the baby kicks the toy pyramid, then the baby will feel pain).

%\textbf{Dataset.} We collected 2400 image data by randomly rotating and positioning the objects used in the environment. For all experiments, we split the data into 2100/300 images and used them for training/testing. 

%Performance of the transferred agent reflects its learning procedure, but also affected by its architecture.
\textbf{Baselines.} Since the performance of the agent is correlated with its architecture, we compare the performance of the agent to baseline agents with the same architecture but different training methods:
\raggedbottom
\begin{itemize}[noitemsep,topsep=0pt,wide,labelindent=0cm,leftmargin=0.35cm]

\item Random : The agent's network is fixed with random initialization and only the connected layer is trained. It shows the naively achievable performance from the architecture.

\item Autoencoder : The agent's network is trained as an autoencoder. We use the performance as a baseline performance of representation learning without explicitly labeled data.

\item Supervised : Both agent's network and the connected network are trained supervised (without transferring). We interpret its performance as an optimal achievable performance with this architecture.

\end{itemize}

%\textbf{Image classification.} Like casual image classification tasks, the agent has to classify images by its included object. We used a linear layer with softmax activation. Additionally, we trained a self-supervised model by using intention as an intrinsic label while exploring the environment.

%\textbf{Distance estimation.} The agent has to estimate the distance between the camera and the object. 
%In other words, the agent has to distinguish the object from the background and estimate its distance. 
%We used 2-layer MLP with ReLU activation for the hidden layer.

%\textbf{Object localization.} The agent has to localize the object with a bounding box. We used 2-layer MLP with ReLU for the hidden layer and designed the network to output center coordinate, width and height of the bounding box.

%\textbf{Implementation Details.} We trained models for 50 epochs using AdamOptimizer with a learning rate of 0.001 for all experiments. We repeated all experiments 5 times and report the average performance. For the intention-based classifier, we maintained a replay buffer with the size of 20000 to mitigate the correlated observation. 


%\textbf{Implementation Details.} We transferred agent's knowledge by fixing the parameters of the agent and connecting additional layers to the interaction features (highlighted with yellow dotted lines in Fig \ref{figure:Agent}). It's worth noting that the number of interaction feature map is extremely small (same as the number of interactions, thus 3 in this experiment), so the agent can't extrapolate its knowledge unless its understanding is compactly stored in the interaction feature map. 

%\textbf{Evaluation Details.} For image classification, we used a linear layer with softmax activation. Additionally, we trained a self-supervised model for image classification with same architecture, but while exploring the environment by using intention as an intrinsic label. To mitigate the correlated observation, we maintained a replay buffer with the size of 20000 and trained with those data. We evaluate this model directly by finding the correspondence between intention and object with the most accuracy without additional training. For depth estimation, we used 2-layer MLP with ReLU activation for the hidden layer.

\subsection{Results and Discussion}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Pictures/WResult_metric.png}
    \caption{Learning curve of transfer learning. For classification and recognition, bigger is better. For distance estimation, smaller is better. Best viewed in color.}
    \label{figure:Agent}
\end{figure*}

\iffalse
\begin{table}[h]
\begin{tabular}{|>{\centering\arraybackslash}m{0.4\textwidth}|>{\centering\arraybackslash}m{0.11\textwidth}|>{\centering\arraybackslash}m{0.11\textwidth}|>{\centering\arraybackslash}m{0.11\textwidth}|>{\centering\arraybackslash}m{0.11\textwidth}|}
\hline
Task (metric)                           & Random & Autoencoder & Proposed & Supervised \\ \hline
Classification (top-1 accuracy)         & 90.0\% & 99.7\%      & 100\%    & 100\%  \\ \hline
Distance estimation (relative L1 error) & 4.01\% & 1.95\%      & 1.62\%   & 0.71\%  \\ \hline
Recognition (intersection of unions)    & 55.2\% & 66.1\%      & 75.1\%   & 87.3\%  \\ \hline
\end{tabular}
\vspace{5px}
\caption{Numerical transfer performance of various models. For classification and recognition, bigger is better. For distance estimation, smaller is better.}
\label{table:Results}
\end{table}
\fi

\begin{table}[h]
\begin{tabular}{|>{\centering\arraybackslash}m{0.32\textwidth}|>{\centering\arraybackslash}m{0.13\textwidth}|>{\centering\arraybackslash}m{0.13\textwidth}|>{\centering\arraybackslash}m{0.13\textwidth}|>{\centering\arraybackslash}m{0.13\textwidth}|}
\hline
Task (Metric, \%)                  & Random & Autoencoder & Proposed & Supervised \\ \hline
Classification (Accuracy)          & 90.0$\pm$2.9  & 99.7$\pm$0.0  & 100$\pm$0     & 100$\pm$0 \\ \hline
Distance estimation (L1 error)     & 4.01$\pm$0.61 & 1.95$\pm$0.08 & 1.62$\pm$0.02 & 0.71$\pm$0.01 \\ \hline
Recognition (IOU)                  & 55.2$\pm$1.2  & 66.1$\pm$0.5  & 75.1$\pm$1.4  & 87.3$\pm$0.8 \\ \hline
\end{tabular}
\vspace{5px}
\caption{Numerical transfer performance with standard errors. For classification and recognition, bigger is better. For distance estimation, smaller is better.}
\label{table:Results}
\end{table}

%We show the classification accuracy of the agent in Table \ref{table:Imageclassification}. We observed that the transferred classifier achieves similar performance with a supervised classifier. 
%As shown in Table \ref{table:Imageclassification}, the transferred classifier could achieve similar performance with a supervised classifier. 
%For the classifier trained by intention, we evaluated the classifier by finding the correspondence between intention and object with the most accuracy. We found that the optimal correspondence maps its intention to the object with the highest reward of applying it, which indicates that the agent could learn the mapping between interaction and objects. However, the accuracy was 76.6\%, which is much lower than the transferred classifier.
%We suppose that it is due to inaccurate labels (the agent might shortly see a pyramid or be heading to the wall while finding an object to kick, but it labels both as a kickable object), and applying memory-based models with temporal information could improve accuracy.
%We suppose that it is due to sporadic inaccurate labels and applying temporal memory-based models could improve accuracy.

%\begin{table}[h]
%\begin{tabular}{|>{\centering\arraybackslash}m{0.1\textwidth}|>{\centering\arraybackslash}m{0.09\textwidth}|>{\centering\arraybackslash}m{0.1\textwidth}|>{\centering\arraybackslash}m{0.09\textwidth}|}
%\hline
%Model    & Random & PlayRoom & Trained \\ \hline
%Relative L1 error    & 0.414   & 0.128   & 0.091    \\ \hline
%\end{tabular}
%\vspace{0px}
%\caption{MSE loss of distance estimation.}
%\label{table:DistanceEstimation}
%\end{table}


%\textbf{Distance Estimation.} Relative absolute error of estimation is shown in Table \ref{table:DistanceEstimation}, which shows that the agent could roughly estimate the distance. However, this isn't trivial since the agent is enough to learn only how to detect the desired object to maximize its reward. Why the agent would store information about distance? We suppose that this ability comes from the training of the critic (value function). Since the critic has to predict the cumulative reward, the agent would learn how much time will be required to reach the object, thus roughly estimate the distance to the object.


%\textbf{Object localization.} IOU accuracy of localization is shown in Table \ref{table:ObjectLocalization}. It shows that the agent was able to estimate the size and position of the object. 

As shown in Table \ref{table:Results}, the transferred models achieved better performance than random and autoencoder models, while being also comparable to supervised models. In specific, the proposed model was able to achieve relative improvement of 0.3\%, 16.9\%, 13.6\% for classification, distance estimation, recognition, from autoencoder models. It shows that the agent was able to learn task-agnostic knowledge from the environment without any explicit labels.

Why the agent would learn those features? For the classification and recognition, we suppose that it is because the agent must recognize and classify the objects to achieve maximal reward, while action of the agent is dependent on the transferred feature. 
For the distance estimation, we suppose that this ability comes from the training of the critic (value function). Since the critic has to predict the cumulative reward, the agent would learn how much time will be required to reach the object, thus roughly estimate the distance to the object.

==> Sections-backup/5_Conclusion.tex <==
\section{Conclusion \& Future Works}
%Inspired from Piaget's theory, we want to see whether understanding of objects could be gained during exploring and interacting with the environment, and also could be extrapolated to other tasks. So we designed an environment which the agent can walk around and interact with objects, and let the agent to explore the environment. After the exploration, we try to extrapolate those knowledge via transfer learning to other computer vision tasks. We observed that transfered models was able to achieve comparable performance with supervised methods, which indicates that the agent was able to gain expandable understanding of object during exploration and interaction.

Inspired from toddler's learning procedure, we proposed a learning procedure which can gain understanding of objects by exploring and interacting with the environment. We evaluated its generality by applying transfer learning to other computer vision tasks. Evaluation results show that the agent was able to gain an expandable understanding of objects by exploring and interacting with the environment. 

However, our method is still far from how a toddler learns. We used hand-crafted reward and applied conventional reinforcement learning algorithm to train the agent. We suggest that substituting hand-crafted reward to intrinsic reward and developing a human-like fast and adaptive learning algorithm would be a promising future direction.

==> Sections/2_Background.tex <==
\section{Background}

\subsection{Related works}
%\hs{Where is current SOTA RL heading? What is the difference of current RL and human intelligence, and the limitation from it?}
%Deep reinforcement learning(DRL) applies deep learning techniques in reinforcement learning framework, showing a great performance in various domains like game theory, optimal control and multi-agent system. Representative algorithms leading these advances are Policy gradient and Deep Q-learning methods.
 % what are the cons of supervised learning?
 % What are the pros of human-like learning / toddler-like learning?
 % Human-like machine learning: limitations and suggestions


%Supervised learning has fundamental limitations in reaching the level of human intelligence despite its advances in fields like computer vision. Firstly, it requires a huge well-labeled dataset to learn a concept or a task, whereas a human can learn with few observations~\cite{lake2017buildingmachines}. It works on the assumption that the dataset is representative, large enough and covers all possible cases~\cite{DBLP:journals/corr/abs-1811-06052} which is in some cases impracticable in domains like medical imaging or activity recognition. Moreover, supervised learning-based algorithms are highly task-specific in the sense that they are optimized well for a single task, but gets trouble in solving multiple tasks~\cite{lake2017buildingmachines}. An agent should at least be able to fit similar tasks with little data to reach the level of artificial general intelligence(AGI). 

%\hs{What is a current limitation of RL, and AI broadly, which will need a human-like learning point-of-view to solve it?}

\iffalse
\textbf{Transferring methods.}
e.g. Meta-learning, Transfer learning, domain adaptation
Need tasks that are in similar domain, well-labeled, easily trainable.

\textbf{Unsupervised methods.}

e.g. XXX-Autoencoder, k-means
Does not work well : lack of inductive bias = poor representation(no difference with compression)
\fi

Attempts to narrow these major discrepancies 
cannot alleviate both of them due to their own limitations. 
Semi-supervised learning trains the predictor given both the labeled data and extra unlabeled data to reduce the cost of labeling.
However, theoretical analysis has found that it increases sample complexity only by a constant factor compared to supervised learning without strong assumption on unlabeled data~\cite{lu2009semisupervisedlearning}.
%suggestive links to the learning in psychology
%~\cite{botvinick2019RLfastandslow}. 
%Data augmentation,
%Simulation-based data synthesis
%Episodic memory, storing records of past events and reusing it to overcome the sample inefficiency, resembles instance-based theories of learning in psychology.
%multitask learning,
% Need to 
%~\cite{logan1988instancebased}.
%In particular, meta learning, term originated from 'learning to learn' in psychology,~\cite{harlow1949learningtolearn}
Meta-learning trains in a set of tasks (usually well-known or general) and leverages the acquired knowledge or configuration in learning a similar task. 
%It does not solve the limitation of supervised learning because there should be sufficient number of well-labeled prior tasks much similar to the target task~\cite{kang2018transferablemetalearning}. 
Still, there should be a sufficient number of well-labeled prior tasks much similar to the target task~\cite{kang2018transferablemetalearning}.
Multi-task learning effectively adapts to a set of related tasks simultaneously by forming an inductive bias from intrinsic dependencies of tasks, but it is difficult to optimize shared parameters in competing objectives of each task~\cite{liu2019multitasklearningauxilarytask}.
%Also, prevailing model-agnostic meta learning(MAML) approaches even assumes simple and concentrated prior task distribution~\cite{vuorio2019multimodalmaml}, which needs further supervision of the developer.

%autonomous learning,

%Semi-supervised learning, self-supervised learning, unsupervised learning, task-agnostic reinforcement learning

%Term was introduced from a psychology domain, that a strong prior knowledge learnt from a specific task are applied in learning a new related task. 
% reward plane 이 gradient descent 에 의해서 수렴이 보장되는 (convex느낌) 걸로 해야된다
% sample inefficiency
% 아키텍쳐간의 비교 : 옆에 supervised 붙이는 아키텍쳐랑 그냥 rl input으로 두 이미지 concat해서 넣은 다음에 intention 없이 줘서 알아서 intention 형성되게하는 구조 
\subsection{How Toddlers Learn}
%Even though recent biologically inspired advances in AI prevails in tasks which were thought only for the human, they are

%\hs{What is a human-like learning and why do you need human-like learning to solve current limitations?}

%\hs{Why can the human-like learning provide a breakthrough to these limitations that other approaches like meta-learning cannot?}
To 
%overcome the limitations of supervised learning and 
build a machine that learns like a human, we need to fuse the human learning process to current AI techniques.
There is a basic difference between data-driven AI and human intelligence in the model of how they learn~\cite{lake2017buildingmachines}. Data-driven AI takes a statistical pattern recognition-based approach, so the accumulation of knowledge relies on the observed data. 
% Prof.Zhang paper i have cited below
In contrast, human actively inspects the environment to collect data and learns with only a few of it by building a generalized model of the world.% to understand them. %~\cite{lake2017buildingmachines}.
%Human-like learning~\cite{DBLP:journals/corr/abs-1811-06052} introduced bio-inspired self-driven data collection in simulation environment to overcome data availability issue in activity recognition. 
%Another attempts tried to mimic human cognition by building an artificial theory-of-mind~\cite{winfield2018TOMexperiments,rabinowitz2018TOMNet,gorur2017TOMSocialRobot} which is the ability to attribute mental states (intentions, desires) of others. However, they was criticized for simplifying the cognitive task into merely a behavioral prediction, rather than actually attributing mental states of others~\cite{shevlin2019PsychologyTermsinAI}.

%, and should take care when analyzing artificial intelligence in an psychological perspective .

% Byungtak Jhang. 2018. Human Intelligence and Machine Intelligence: Cognitive Artificial Intelligence (in Korean). Communications of KIISE 36, 1 (2018), 17–26.
% How do we cite this korean article?
%A promising direction to overcome such differences is constructing cognitive agents that imitate human-like perceptions and mental process. some works report that cognition is highly correlated with performing actions and having rich perceptions. Reflecting how human learn, cognitive agent aims at learning task-independent knowledge by continuously observing environment with various sensory perceptions and solving generic tasks. There have been early discussions in robotics and computer science of building cognitive agents~\cite{lee2017cognitiveagentearlywork}.

The learning process of a child is important for learning-to-learn capabilities like goal-setting, self-control~\cite{zosh2017learnthruplayreview}, and should be taken into account in developing AGI. Life experiences and prior knowledge learnt in childhood are known to influence the learning of a grown-up.
%Importance of childhood learning has thus raised attention to computer scientists like Turing or Schank~\cite{turing2009child,schank1972nlp} aiming to model the AGI. 
%Instead of building a machine imitating adult mind, Turing suggested to build a child mind and educating it~\cite{turing2009child}. Schank has also made a prospect of a program expanding their knowledge like a child, instead of catered in tremendous data~\cite{schank1972nlp}.
The latest works in deep learning like visual object learning~\cite{bambach2018toddlerinspiredvisualobject} 
%or few-shot learning~\cite{ritter2017cognitivepsyonDNN} 
are seeking advance from how children learn. 
%Data collected from toddler-like visual system is used to train visual object learning better, or one-shot learning image classification model shows a similar shape bias as children.

%\hs{What is the difference of toddler and adult human being and what can be inspired from the toddler's learning?}
Researches in developmental psychology suggest that toddler unconsciously learns through interaction and play with their surrounding environment, rather than self-directed task-specific learning of an adult~\cite{mcdonough2013difference_adult_child}. Too early the start of formal subject teaching for a child is known to be counterproductive and hinders academic performance in the long run~\cite{suggate2013childlatelearning}. Instead, it is universally accepted that children learn cognitive or self-regulatory abilities by playing~\cite{piaget1952origins,zosh2017learnthruplayreview}.
%Piaget viewed that toddler builds much abstract and symbolized model of the surrounding world through playing.
%, and a new kind of psychological functioning emerges.
%playing increases in the developmental stage of a toddler (preoperational stage) in order to~\cite{piaget1952origins}.
%However, playing of toddler is usually not self-directed, but more like a random interaction with the environment.
%Adult learners have more self-directed nature of learning process to formulate a learning goal due to their prior knowledges whereas child learners is less self-directed and more unconscious of their learning process~\cite{mcdonough2013difference_adult_child}.
Large-scale studies on exploratory object manipulation in early childhood has found that changes from random actions on objects to more self-directed and functional activities happen at the latter part of the first years of a child~\cite{gibson1988toddlerlearning}. Random actions in the early exploration are suggested as investigating an object with the raw sensory-perceptual feedback, with visuotactile inspection like mouthing, chewing, rotating, banging and else. These activities promote the development of cognitive capacities and control and progress to more functional and imaginative plays like talking to a toy telephone. It gives an inspiration that action-based exploration of a toddler can facilitate an unsupervised categorization of the objects, and furthermore, help gain a general knowledge of the world that can be used to adapt to a specific task.

%both adults and children need to use the learning or employ the knowledge gained. The more the knowledge is used, the closer the approximations come to the conventions and become internalized. Feedback to both the adult and the child helps each learner fine tune the approximations. Once the learning has been internalized, the knowledge is transferred into new situations by both the adult and child learners. A major characteristic that impacts the natural learning process is engagement of both adult and child learners. The more actively engaged in the learning process, the faster the knowledge is obtained and the better the knowledge is learned. 
% 이부분정리해야함
%In the 1970s the literature of early childhood was enriched by large-scale studies of exploratory manipulation of objects (e.g. McCall 1974; Fenson et al 1976). The relevant concept that inspired these studies was cognition, as the study of cognitive development emerged with the new focus on cognitive psychology. Emphasis was placed on a change toward the end of the first year of a child's life from relatively random action on objects, to cognitively directed "functional" activities, such as drinking from a toy cup or talking into a toy telephone instead of banging them on somelhing. McCall suggested that early exploration was "largely an investigation of the raw sensory-perceptual feedback of the objects" (1974, p. 77), which changed progressively toward greater cognitive control and imaginative play with the object. Fenson et al (1976) similarly stressed emergence of new "cognitive capacities" following nonspecific manipulation: Although 9-month-olds generally showed the ability to relate to objects and 7-month-olds did not, at both ages play was nonrelational and nonaccommodative and was characterized by close visual and tactual inspection of individual objects, usually accompanied bymouthing and chewing and the application of more or less indisciminate motor schemes
%(shaking, banging, turning the object over and over, and shifting it from hand to hand) ....The emergence of relational acts in the latter part of the first year and the emergence of symbolic acts in the first half of the second year dramatically change the structure of the child's play, mirroring the development of important new cognitive capacitis (pp. 234 ff).It is interesting to read that the play mirrors the development of new cognitive capacities, rather than that the manipulative play has a key role in cognitive development, as Piaget would have suggested. 

%\hs{What are you actually trying to do? formulate it clearly please.}
%world exploration

%\hs{How does this represent the human-like learning?}
%\hs{How is it different from meta-learning?}
%\hs{What is the problem and why are you trying to solve in this way?}
%\hs{How is human-like learning applied in your implementation? }
%\hs{ Why are you using a navigation task to demonstrate the human-like learning?}

